Towards multi-sequence MR image recovery from undersampled k-space data

Undersampled MR image recovery has been widely studied for accelerated MR acquisition. However, it has been mostly studied under a single sequence scenario, despite the fact that multi-sequence MR scan is common in practice. In this paper, we aim to optimize multi-sequence MR image recovery from undersampled k-space data under an overall time constraint while considering the difference in acquisition time for various sequences. We first formulate it as a constrained optimization problem and then show that finding the optimal sampling strategy for all sequences and the best recovery model at the same time is combinatorial and hence computationally prohibitive. To solve this problem, we propose a blind recovery model that simultaneously recovers multiple sequences, and an efficient approach to find proper combination of sampling strategy and recovery model. Our experiments demonstrate that the proposed method outperforms sequence-wise recovery, and sheds light on how to decide the undersampling strategy for sequences within an overall time budget.

==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/ablation/ablation_1st_img.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}

\begin{tabularx}{\textwidth}{ *{4}{Y} }
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF2_4_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        %\caption{$3\times t_{T1} = 2\times t_{T2} = t_{FLAIR}$}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF1_71_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF1_6_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        %\caption{$3\times t_{T1} = 2\times t_{T2} = t_{FLAIR}$}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF2_67_crop.png}
    \end{subfigure}\\
    
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_111_SF2_4_crop.png}
        \caption{$42\%$ time saved}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_111_SF1_71_crop.png}
        \caption{$58\%$ time saved}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_123_SF1_6_crop.png}
        \caption{$37.5\%$ time saved}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_123_SF2_67_crop.png}
        \caption{$62.5\%$ time saved}
    \end{subfigure}
\end{tabularx}
\caption{Comparison of performances of simultaneous reconstruction between BRM ($f_\theta$) and $f^{\mathcal{M}_{1:S}}_\theta$. The choices of $\mathcal{M}_{1:S}$ are listed along the $x$ axis, in the order of [$T_1$, $T_2$, FLAIR] downsampling factors. `ZF' means reconstruction using the undersampled k-space that is zero-filled. }\label{fig:ablation_1st}
\end{figure*}    

==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/ablation/new_table_graph.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[t!]
\small
\begin{tabular}{ |c|c|c|c| }
% \begin{tabularx}{\textwidth}{ |c|c|c|c|c|c} 
\hline
\multicolumn{4}{|c|}{$t_{T_1}$:$t_{T_2}$:$t_{flair}$}\\
\hline
\multicolumn{2}{|c|}{1:1:1}
& \multicolumn{2}{c|}{2:3:6}
\\
\hline
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF1_71_good_crop.png}
    \end{subfigure} 
 & 
     \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF2_4_good_crop.png}
    \end{subfigure} 
 & 
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF1_6_good_crop.png}
    \end{subfigure}
 &
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF2_67_good_crop.png}
    \end{subfigure}

 \\
 \hline
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_111_SF2_4_crop.png}
        \caption{$42\%$ time saved}
    \end{subfigure}
 & 
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_111_SF1_71_crop.png}
        \caption{$58\%$ time saved}
    \end{subfigure}
 & 
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_123_SF1_6_crop.png}
        \caption{$37.5\%$ time saved}
    \end{subfigure}
 &
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_123_SF2_67_crop.png}
        \caption{$62.5\%$ time saved}
    \end{subfigure}
 \\

\hline

\end{tabular}
\vspace{2pt}

\caption{Comparison of performances of simultaneous reconstruction between BRM ($f_\theta$) and $f^{\mathcal{M}_{1:S}}_\theta$. The choices of $\mathcal{M}_{1:S}$ are listed along the $x$ axis, in the order of [$T_1$, $T_2$, FLAIR] downsampling factors. `ZF' means reconstruction using the undersampled k-space that is zero-filled. }\label{fig:ablation_1st}
\vspace{-0.5cm}
\end{figure*}  

==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/graph/graph.tex <==

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[t!]
\captionsetup[subfigure]{labelformat=empty}
\begin{tabularx}{\textwidth}{ |*{6}{Y}| }
\hline

Sequence& LR & SISO & MIMO & MIMO tuned & GT \\
\hline
 $\lambda_{T_1} = 6.63$ &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_0_LR.png}
    \vspace{-2em}
    \caption{\tiny{34.38/0.9371}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/SISO_1_7_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{42.42/0.9883}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{44.60/0.9920}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/tuned_1_7_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{{\bf 45.50}/{\bf 0.9940}}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_0_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{T_2} = 2.11$ &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_1_LR.png}
    \vspace{-2em}
    \caption{\tiny{29.74/0.8903}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/SISO_1_7_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{36.25/0.9734}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{36.42/0.9752}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/tuned_1_7_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{{\bf 37.70}/{\bf 0.9832}}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_1_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{flair} = 8.00$ &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_2_LR.png}
    \vspace{-2em}
    \caption{\tiny{39.89/0.9311}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/SISO_1_7_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{43.94/0.9864}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{44.74/0.9883}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/tuned_1_7_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{{\bf 45.49}/{\bf 0.9894}}}
\end{subfigure} &
\begin{subfigure}[t]{0.12\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111/1_7_2_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
\end{tabularx}
\vspace{-1em}
\caption{Visual comparison of different methods, with PSNR (dB) and SSIM values listed under the images. After recovery, the images are shaper with more visible details.}\label{fig:vis}
%\vspace{0.2cm}
\vspace{-1.5em}
\end{figure*}



==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/graph/simulated_graph.tex <==

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[!htb]
\captionsetup[subfigure]{labelformat=empty}
\begin{tabularx}{\textwidth}{ |*{6}{Y}| }
\hline

Sequence& LR & SISO & MIMO & MIMO tuned & GT \\
\hline
 $\lambda_{T_1} = 2.61$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/LR_0_crop.png}
    \vspace{-2em}
    \caption{\tiny{34.25/0.9423}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_T1_crop.png}
    \vspace{-2em}
    \caption{\tiny{39.24/0.9701}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_0_BRM_crop.png}
    \vspace{-2em}
    \caption{\tiny{40.68/0.9821}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_0_TUNED_crop.png}
    \vspace{-2em}
    \caption{\tiny{{\bf41.19}/{\bf0.9840}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/HR_0_crop.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{T_2} = 3.74$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/LR_1_crop.png}
    \vspace{-2em}
    \caption{\tiny{31.80/0.9061}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_T2_crop.png}
    \vspace{-2em}
    \caption{\tiny{33.10/0.9687}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_1_BRM_crop.png}
    \vspace{-2em}
    \caption{\tiny{33.46/0.9716}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_1_TUNED_crop.png}
    \vspace{-2em}
    \caption{\tiny{{\bf33.59}/{\bf0.9739}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/HR_1_crop.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{flair} = 5.16$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/LR_2_crop.png}
    \vspace{-2em}
    \caption{\tiny{28.23/0.8227}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_FLAIR_crop.png}
    \vspace{-2em}
    \caption{\tiny{30.34/0.9301}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_2_BRM_crop.png}
    \vspace{-2em}
    \caption{\tiny{32.84/0.9396}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/SR_2_TUNED_crop.png}
    \vspace{-2em}
    \caption{\tiny{{\bf35.37}/{\bf0.9448}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_123/HR_2_crop.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
\end{tabularx}
\caption{Visual comparison of different recovery methods on simulated data. Note that BraTS sequences are interpolated for registration; therefore the image quality is not as good as the real data.}
\end{figure*}



==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/graph/simulated_graph_supp2.tex <==

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[!htb]
\captionsetup[subfigure]{labelformat=empty}
\begin{tabularx}{\textwidth}{ |*{6}{Y}| }
\hline

Sequence& LR & SISO & MIMO & MIMO tuned & GT \\
\hline
 $\lambda_{T_1} = 5.66$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_0_LR.png}
    \vspace{-2em}
    \caption{\tiny{27.13/0.7916}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_sing_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{33.91/0.8953}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{34.60/0.9111}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_tune_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{34.90}/\bf{0.9225}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_0_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{T_2} = 3.14$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_1_LR.png}
    \vspace{-2em}
    \caption{\tiny{29.19/0.9016}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_sing_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{37.06/0.9667}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{36.73/0.9619}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_tune_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{37.62}/\bf{0.9671}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_1_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{flair} = 3.39$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_2_LR.png}
    \vspace{-2em}
    \caption{\tiny{26.51/0.8290}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_sing_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{34.58/0.9221}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{34.59/0.9252}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_tune_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{35.11}/\bf{0.9340}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_sim/img2_2_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
\end{tabularx}
\caption{Visual comparison of different recovery methods on simulated data}
%\vspace{0.2cm}
%\vspace{-0.8cm}
\end{figure*}



==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/graph/simulated_graph_supp3.tex <==

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[!htb]
\captionsetup[subfigure]{labelformat=empty}
\begin{tabularx}{\textwidth}{ |*{6}{Y}| }
\hline

Sequence& LR & SISO & MIMO & MIMO tuned & GT \\
\hline
 $\lambda_{T_1} = 6.63$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_0_LR.png}
    \vspace{-2em}
    \caption{\tiny{35.46/0.9431}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/SISO_6_13_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{40.82/0.9826}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{41.84/0.9857}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/tune_6_13_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{42.12}/\bf{0.9867}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_0_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{T_2} = 2.11$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_1_LR.png}
    \vspace{-2em}
    \caption{\tiny{32.34/0.9254}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/SISO_6_13_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{36.19/0.9699}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{36.42/\bf{0.9711}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/tune_6_13_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{36.78}/0.9695}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_1_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{flair} = 8.00$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_2_LR.png}
    \vspace{-2em}
    \caption{\tiny{42.54/0.9489}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/SISO_6_13_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{45.24/0.9837}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{45.89/0.9868}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/tune_6_13_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{46.35}/\bf{0.9880}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img_111_extra/6_13_2_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
\end{tabularx}
\caption{Visual comparison of different recovery methods on real data}
\end{figure*}



==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/graph/simulated_graph_supp4.tex <==

\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[!htb]
\captionsetup[subfigure]{labelformat=empty}
\begin{tabularx}{\textwidth}{ |*{6}{Y}| }
\hline

Sequence& LR & SISO & MIMO & MIMO tuned & GT \\
\hline
 $\lambda_{T_1} = 2.90$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_0_LR.png}
    \vspace{-2em}
    \caption{\tiny{38.30/0.9484}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/SISO_6_9_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{45.03/0.9920}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{45.35/0.9926}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/tune_6_9_0_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{46.70}/\bf{0.9951}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_0_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{T_2} = 2.44$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_1_LR.png}
    \vspace{-2em}
    \caption{\tiny{29.78/0.8990}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/SISO_6_9_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{35.43/0.9720}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{35.93/0.9752}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/tune_6_9_1_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{37.05}/\bf{0.9809}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_1_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
 $\lambda_{flair} = 7.82$ &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_2_LR.png}
    \vspace{-2em}
    \caption{\tiny{41.24/0.9412}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/SISO_6_9_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{44.54/0.9850}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{45.66/0.9885}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/tune_6_9_2_SR.png}
    \vspace{-2em}
    \caption{\tiny{\bf{46.15}/\bf{0.9891}}}
\end{subfigure} &
\begin{subfigure}[t]{0.125\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graph/img146/6_9_2_HR.png}
    \vspace{-2em}
    \caption{\tiny{PSNR/SSIM}}
\end{subfigure}\\ 
\hline
\end{tabularx}
\caption{Visual comparison of different recovery methods on real data}
%\vspace{0.2cm}
%\vspace{-0.8cm}
\end{figure*}



==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/lambda_space_graph/lambda_space.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}

\begin{tabularx}{\textwidth}{ *{2}{Y} }
    \begin{subfigure}[t]{0.5\textwidth}
        \caption{$t_{T_1}:t_{T_2}:t_{flair}$=1:1:1}
        \centering
        \includegraphics[width=\linewidth]{lambda_space_graph/sSRvsSR_by_var_111_label_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.5\textwidth}
        \caption{$t_{T_1}:t_{T_2}:t_{flair}$=2:3:6}
        \centering
        \includegraphics[width=\linewidth]{lambda_space_graph/sSRvsSR_by_var_123_crop.png}
    \end{subfigure}
\end{tabularx}
\caption{Quantitative reconstruction performance comparison between SISO and MIMO models. The $x$ axis is sorted by the variance of $\{\lambda_s\}^S_{s=1}$ from the largest to the smallest, which is 0.} \label{fig:lambda_space}
\end{figure*}    

==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/lambda_space_graph/tune_table.tex <==

\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[t!]

\small
\begin{tabularx}{\textwidth}{ |Y|c|*{6}{Y|} }
% \begin{tabularx}{\textwidth}{ |c|c|c|c|c|c} 
\hline
$t_{T_1}$:$t_{T_2}$:$t_{flair}$ & $\lambda_{T_1}, \lambda_{T_2}, \lambda_{flair}$ & ZF & SISO & MIMO & MIMO (tuned)\\
\hline

$1:1:1$ & 6.6, 2.1, 8.0 &33.48/0.918 & 38.57/0.980 & 39.24/0.984 & 40.00/0.987  \\
Real & 8.00, 2.11, 6.63 &33.43/0.920 & 38.36/0.979 & 39.16/0.984 & {\bf 40.07}/{\bf 0.987} \\
 & 7.25, 2.11, 7.25 &33.39/0.918 & 38.50/0.980 & 39.15/0.984 & 40.07/0.986\\

\hline
$1:4:6$ & 2.90, 2.44, 7.82 & 33.81/0.926 & 38.85/0.983 & 39.33/0.985 & 40.28/0.988\\
Real & 3.01, 2.44, 7.69 & 33.60/0.924 & 38.83/0.983 & 39.32/0.985 & {\bf 40.37}/{\bf 0.987}\\
 & 3.93, 2.44, 6.99 & 33.58/0.925 & 38.81/0.983 & 39.31/0.986 & 40.13/0.987\\
\hline
$1:1:1$ & 5.66, 3.14, 3.93 &32.21/0.887 & 37.69/0.974 & 38.32/0.978 & {\bf 38.99}/{\bf 0.980}  \\
Simulated & 5.27, 3.41, 3.74 &32.31/0.889 & 37.88/0.975 & 38.31/0.979 & 38.98/0.980 \\
 & 6.10, 3.14, 3.74 &32.21/0.887 & 37.51/0.973 & 38.31/0.978 & 38.99/0.980\\

\hline
 $2:3:6$ & 2.61, 3.74, 5.16 &32.87/0.899 & 38.01/0.976 & 38.67/0.980 & {\bf 39.37}/{\bf 0.982}  \\
 Simulated& 2.44, 3.74, 5.40 & 32.84/0.899& 37.87/0.975 & 38.66/0.980 & 39.35/0.982 \\
 & 2.61, 3.41, 5.66 &32.82/0.899 & 37.80/0.975 & 38.65/0.980 & 39.33/0.982\\
\hline

\end{tabularx}
\vspace{2pt}
\caption{Quantitative evaluations for the top performing $\lambda_{1:S}$ under different acquisition time assumption. The performance numbers presented here are PSNR (dB) and SSIM. }
\label{tab:Comparison}
\vspace{-2.5em}
\end{table*}

==> Towards multi-sequence MR image recovery from undersampled k-space data (1)/old_text.tex <==

\iffalse
\section{Problem Formulation}
We first note that the most popular MR k-space sampling method is through Cartesian trajectory, where a series of acquisition is performed along parallel equispaced lines, which is conventionally called {\em phase encodes}. This leads to a natural implementation for MR undersampling, where the technicians can drop certain phase encodes from the sampling grid\cite{lustig2007sparse}. In this paper, we focus on undersampling with 1D masks along the phase encode direction. There are other possible sampling trajectories and undersampling patterns; however, they are less popular, and will not be the focus here. For those scenarios, the overall formulation still stands true and only needs slight modification. 

Consider multiple MR sequences indexed by $s \in \{1,2,...,S\}$ and assume that all sequences are sampled from a k-space with $N$ phase encodes. For each sequence $s$, the unit time for sampling a phase encode is denoted by $t_s$ and the number of lines by $n_s$. For full sampling, $n_s=N$; for undersampling, $n_s<N$ with a sparsity factor $\lambda_s = N/n_s$.
The total amount of time for sampling the k-space of all sequences is 
\begin{equation}
T=\sum_{s=1}^{S} t_{s}\times n_s = \sum_{s=1}^{S} \frac{t_{s} \times N} {\lambda_s}
\end{equation}
It is obvious that the time need for full sampling of all sequence is
\begin{equation}
T_{full}=\sum_{s=1}^{S} t_{s}\times N
\end{equation}

We further define the maskings $\mathcal{G}_s\colon{\mathbb{N}}\to{\{0,1\}^{N\times N}}$, which yield undersampling patterns based on the available $n_s$. We can then define the undersampled MR image for every sequence to be

\begin{equation}
I^{\mathcal{G}_s}_{\downarrow \lambda_s} = \mathcal{F}^{-1}(\mathcal{G}_s(\frac{N}{\lambda_s}) \odot F_s) = \mathcal{F}^{-1}(\mathcal{G}_s(n_s) \odot F_s)
\end{equation}
where $F_s$ denotes the full k-space spectrum of a given sequence, and $\mathcal{F}^{-1}$ denotes the inverse fourier transform.
The set of images reconstructed from undersampled k-space data are denoted by 
$I^{\mathcal{G}_{1:S}}_{\downarrow \lambda_{1:S}}=\{I^{\mathcal{G}_s}_{\downarrow \lambda_s}\}_{s=1}^S$. 
For full sampling with $\lambda_s=1$, we have $I_{1:S}=\{I_s\}_{s=1}^S$ with $I_s = I_{\downarrow (\lambda_s=1)}$.

Ideally, we aim to learn a model $\mathcal{M_{\theta}}$ that offers a recovery of $\{I_s\}_{s=1}^S$ from $\{I^{\mathcal{G}_{1:S}}_{\downarrow \lambda_{1:S}}\}_{s=1}^S$ via minimizing the expected reconstruction loss {\em under a time constraint}.
\begin{align} \label{eq:recovery}
    \min_{\mathcal{M_{\theta}},\lambda_{1:S},\mathcal{G}_{1:S}}~~  \mathcal{L}_{recon} = \mathcal{E}_{p(I_{1:S})}[\mathcal{L}( \mathcal{M_{\theta}}(I^{\mathcal{G}_{1:S}}_{\downarrow \lambda_{1:S}})~,~I_{1:S})] \\ 
    \text{s.t.}~T= \sum_{s=1}^{S} \frac{t_{s} \times N} {\lambda_s} ~ \le T_{budget} = \frac{T_{full}}{\lambda}, \nonumber
\end{align}
where $\mathcal{E}$ takes expectation over the images $I_{1:S}$ recovered from fully sampled data, $\mathcal{L}(\cdot,\cdot)$ is a loss function (say the $L_1$ loss we empirically use),  $T_{budget}$ is a given time budget, and $\lambda=T_{full}/T_{budget}$ is an overall time saving factor.

Unfortunately, directly solving the problem in (\ref{eq:recovery}) is challenging as it contains three subproblems related to (i) recovery model (RM), (ii) sampling ratio (SR), and (iii) sampling pattern (SP).
Specifically, 
\begin{itemize}
    \item 
The first RM subproblem is to select the right model $\mathcal{M}$ and optimize its associated parameter $\theta$, given a fixed sampling strategy with $\lambda_{1:S}$ and $\mathcal{G}_{1:S}$ known.
\item 
The second SR subproblem is to pick the right sampling ratio, that is, solving for $\lambda_{1:S}$ given a known model $\mathcal{M_{\theta}}$ and the best sampling pattern $\mathcal{G}_s$ for each sequence. In practice, choosing the right SR may also depend on the importance of each sequence with regards to specific diseases.
\item
The third SP subproblem is to select the right sampling pattern. Given a known model $\mathcal{M_{\theta}}$ and the desirable sampling ratios $\lambda_{1:S}$, we want to find the optimally efficient sampling pattern $\mathcal{G}_{1:S}$ that leads to the most information recovered for each sequence. 
\end{itemize}
To complicate the matter, the three subproblems are mixed together. The optimal recovery model depends on the sampling strategy and vice verse, while the best sampling pattern may be different for every sequence, under its specific sampling ratio.

In this paper, we make preliminary attempts with simplifying assumptions and empirical findings to solve these three subproblems. While we will touch on the effect of different SPs, the main focus of this paper will be on finding the best RM and SR with a pre-determined SP. 
%In general, we use sampling strategy (SS) as an umbrella term to mean variable SR and fixed SP. 



\subsection{Recovery network}
We use deep neural network (NN) as our choice for RM $\mathcal{M_{\theta}}$. Since the RM takes multiple images from different sequences as inputs, one has the choice of training (a) multiple individual NNs, one per sequence, or (b) one simultaneous, monolithic NN for all sequences. 

As mentioned above, the right RM choice might depend on the specific SR; however, we hypothesize that such an RM choice is independent of SR. This is realized by learning an RM that is insensitive to the SR. In other words, during the process of learning an RM, we take a data augmentation approach: for each training data point, we associate it with a random choice of $\lambda_{1:S}$.
We can then empirically verify which RM, individually or simultaneously learned, yield the smaller loss. 
\begin{align} \label{eq:RM}
    \min_{\mathcal{M_{\theta}} \in \mathcal{Z}}~~  \mathcal{L}_{recon} = \mathcal{E}_{p(I_{1:S},\lambda_{1:S})}[\mathcal{L}( \mathcal{M_{\theta}}(I_{\downarrow \lambda_{1:S}})~,~I_{1:S})],
\end{align}
where $\mathcal{Z}$ is the model zoo of interest and $\mathcal{E}$ takes expectation over the images $I_{1:S}$ recovered from fully sampled data and the sparsity factors $\lambda_{1:S}$. We denote the minimizing RM as $\tilde{\mathcal{M_{\theta}}}$.

\subsection{Sampling strategy}

Given the RM $\tilde{\mathcal{M_{\theta}}}$ learned in an SS-insensitive fashion and assuming that the sparsity factor $\lambda_s$ takes a value in a discrete set $\Lambda=\{\hat{\lambda}^1,\hat{\lambda}^2,...,\hat{\lambda}^F\}$, it is possible to find the optimal SS via exhaustive search. 

\begin{align} \label{eq:SS}
    \min_{\lambda_{1:S} \in \Lambda}~~  \mathcal{L}_{recon} = \mathcal{E}_{p(I_{1:S})}[\mathcal{L}( \tilde{\mathcal{M_{\theta}}}(I_{\downarrow \lambda_{1:S}})~,~I_{1:S})] \\ 
    \text{s.t.}~T= \sum_{s=1}^{S} \frac{t_{s} \times N} {\lambda_s} ~ \le T_{budget} = \frac{T_{full}}{\lambda}, \nonumber
\end{align}
where $\mathcal{E}$ takes expectation over the images $I_{1:S}$ recovered from fully sampled data.

This is done in two steps for each possible SS configuration.
\begin{itemize}
    \item Step 1: Check if the SS configuration satisfies the time constraint.
    \item Step 2: If it does, then compute its associated reconstruction loss. 
\end{itemize}
Out of all SS configurations that reaches Step 2, we pick the SS configuration that generates the minimal loss.

To further refine the reconstruction quality, we perform one final round of tuning by learning an RM model specific to the selected SS configuration or mutliples RMs corresponding to a list of top SS configurations.
\fi

% \subsubsection{Individual vs Simultaneous reconstruction}

% With many CNN-based MR reconstruction methods focused on single sequence reconstruction, a natural extension for multi-sequence scenario is to learn multiple models $\mathcal{M}_{\theta_1}, \mathcal{M}_{\theta_2},...,\mathcal{M}_{\theta_s}$, each of which focuses on de-alising noise for a specific sequence. In this case, the models together compose $\mathcal{M}_{\theta}$, and the overall reconstruction loss can written as 

% \begin{align}
%     \min_{\theta_s,\lambda_s}  \mathcal{L}_{recon} =  \mathcal{E}[\mathcal{L}(\{ \mathcal{M}_{\theta_s}(I_{\downarrow \lambda_s})\}_{s=1}^S~,~\{I_{s}\}_{s=1}^S)],
% \end{align}

% This formulation does not take into account the shared information across different sequences. As both Xiang et al. \cite{DBLP:conf/miccai/XiangCCZLWS18} and Huang et al. \cite{DBLP:conf/miccai/HuangCA12} have shown, there exist a large amount of correlation between sequences on the same patient, as they share the underlying anatomic structures. Even if some anatomic detail is lost in one sequence due to under-sampling, such information may be present in other sequences. On the other hand, this formulation also leads to training excessive amount of models, as the de-aliasing task is common over all sequences and will lead to network learning similar features. Therefore, it makes much more sense to train one network which has access to all the sequences, and let it learn the best features among them. In practice, 

















==> ablation/ablation_1st_img.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}

\begin{tabularx}{\textwidth}{ *{4}{Y} }
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF2_4_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        %\caption{$3\times t_{T1} = 2\times t_{T2} = t_{FLAIR}$}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF1_71_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF1_6_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        %\caption{$3\times t_{T1} = 2\times t_{T2} = t_{FLAIR}$}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF2_67_crop.png}
    \end{subfigure}\\
    
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_111_SF2_4_crop.png}
        \caption{$42\%$ time saved}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_111_SF1_71_crop.png}
        \caption{$58\%$ time saved}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_123_SF1_6_crop.png}
        \caption{$37.5\%$ time saved}
    \end{subfigure} &
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/ssim_123_SF2_67_crop.png}
        \caption{$62.5\%$ time saved}
    \end{subfigure}
\end{tabularx}
\caption{Comparison of performances of simultaneous reconstruction between BRM ($f_\theta$) and $f^{\mathcal{M}_{1:S}}_\theta$. The choices of $\mathcal{M}_{1:S}$ are listed along the $x$ axis, in the order of [$T_1$, $T_2$, FLAIR] downsampling factors. `ZF' means reconstruction using the undersampled k-space that is zero-filled. }\label{fig:ablation_1st}
\end{figure*}    

==> ablation/new_table_graph.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}[t!]
\small
\begin{tabular}{ |c|c|c|c| }
% \begin{tabularx}{\textwidth}{ |c|c|c|c|c|c} 
\hline
\multicolumn{4}{|c|}{$t_{T_1}$:$t_{T_2}$:$t_{flair}$}\\
\hline
\multicolumn{2}{|c|}{1:1:1}
& \multicolumn{2}{c|}{2:3:6}
\\
\hline
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF1_71_good_crop.png}
    \end{subfigure} 
 & 
     \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_111_SF2_4_good_crop.png}
    \end{subfigure} 
 & 
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF1_6_good_crop.png}
    \end{subfigure}
 &
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.3cm]{ablation/psnr_123_SF2_67_good_crop.png}
    \end{subfigure}

 \\
 \hline
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_111_SF2_4_crop.png}
        \caption{$42\%$ time saved}
    \end{subfigure}
 & 
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_111_SF1_71_crop.png}
        \caption{$58\%$ time saved}
    \end{subfigure}
 & 
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_123_SF1_6_crop.png}
        \caption{$37.5\%$ time saved}
    \end{subfigure}
 &
     \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=2.2cm]{ablation/ssim_123_SF2_67_crop.png}
        \caption{$62.5\%$ time saved}
    \end{subfigure}
 \\

\hline

\end{tabular}
\vspace{2pt}

\caption{Comparison of performances of simultaneous reconstruction between BRM ($f_\theta$) and $f^{\mathcal{M}_{1:S}}_\theta$. The choices of $\mathcal{M}_{1:S}$ are listed along the $x$ axis, in the order of [$T_1$, $T_2$, FLAIR] downsampling factors. `ZF' means reconstruction using the undersampled k-space that is zero-filled. }\label{fig:ablation_1st}
\vspace{-0.5cm}
\end{figure*}  

==> lambda_space_graph/lambda_space.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}

\begin{tabularx}{\textwidth}{ *{2}{Y} }
    \begin{subfigure}[t]{0.5\textwidth}
        \caption{$t_{T_1}:t_{T_2}:t_{flair}$=1:1:1}
        \centering
        \includegraphics[width=\linewidth]{lambda_space_graph/sSRvsSR_by_var_111_label_crop.png}
    \end{subfigure} &
    \begin{subfigure}[t]{0.5\textwidth}
        \caption{$t_{T_1}:t_{T_2}:t_{flair}$=2:3:6}
        \centering
        \includegraphics[width=\linewidth]{lambda_space_graph/sSRvsSR_by_var_123_crop.png}
    \end{subfigure}
\end{tabularx}
\caption{Quantitative reconstruction performance comparison between SISO and MIMO models. The $x$ axis is sorted by the variance of $\{\lambda_s\}^S_{s=1}$ from the largest to the smallest, which is 0.} \label{fig:lambda_space}
\end{figure*}    

==> old_text.tex <==

\iffalse
\section{Problem Formulation}
We first note that the most popular MR k-space sampling method is through Cartesian trajectory, where a series of acquisition is performed along parallel equispaced lines, which is conventionally called {\em phase encodes}. This leads to a natural implementation for MR undersampling, where the technicians can drop certain phase encodes from the sampling grid\cite{lustig2007sparse}. In this paper, we focus on undersampling with 1D masks along the phase encode direction. There are other possible sampling trajectories and undersampling patterns; however, they are less popular, and will not be the focus here. For those scenarios, the overall formulation still stands true and only needs slight modification. 

Consider multiple MR sequences indexed by $s \in \{1,2,...,S\}$ and assume that all sequences are sampled from a k-space with $N$ phase encodes. For each sequence $s$, the unit time for sampling a phase encode is denoted by $t_s$ and the number of lines by $n_s$. For full sampling, $n_s=N$; for undersampling, $n_s<N$ with a sparsity factor $\lambda_s = N/n_s$.
The total amount of time for sampling the k-space of all sequences is 
\begin{equation}
T=\sum_{s=1}^{S} t_{s}\times n_s = \sum_{s=1}^{S} \frac{t_{s} \times N} {\lambda_s}
\end{equation}
It is obvious that the time need for full sampling of all sequence is
\begin{equation}
T_{full}=\sum_{s=1}^{S} t_{s}\times N
\end{equation}

We further define the maskings $\mathcal{G}_s\colon{\mathbb{N}}\to{\{0,1\}^{N\times N}}$, which yield undersampling patterns based on the available $n_s$. We can then define the undersampled MR image for every sequence to be

\begin{equation}
I^{\mathcal{G}_s}_{\downarrow \lambda_s} = \mathcal{F}^{-1}(\mathcal{G}_s(\frac{N}{\lambda_s}) \odot F_s) = \mathcal{F}^{-1}(\mathcal{G}_s(n_s) \odot F_s)
\end{equation}
where $F_s$ denotes the full k-space spectrum of a given sequence, and $\mathcal{F}^{-1}$ denotes the inverse fourier transform.
The set of images reconstructed from undersampled k-space data are denoted by 
$I^{\mathcal{G}_{1:S}}_{\downarrow \lambda_{1:S}}=\{I^{\mathcal{G}_s}_{\downarrow \lambda_s}\}_{s=1}^S$. 
For full sampling with $\lambda_s=1$, we have $I_{1:S}=\{I_s\}_{s=1}^S$ with $I_s = I_{\downarrow (\lambda_s=1)}$.

Ideally, we aim to learn a model $\mathcal{M_{\theta}}$ that offers a recovery of $\{I_s\}_{s=1}^S$ from $\{I^{\mathcal{G}_{1:S}}_{\downarrow \lambda_{1:S}}\}_{s=1}^S$ via minimizing the expected reconstruction loss {\em under a time constraint}.
\begin{align} \label{eq:recovery}
    \min_{\mathcal{M_{\theta}},\lambda_{1:S},\mathcal{G}_{1:S}}~~  \mathcal{L}_{recon} = \mathcal{E}_{p(I_{1:S})}[\mathcal{L}( \mathcal{M_{\theta}}(I^{\mathcal{G}_{1:S}}_{\downarrow \lambda_{1:S}})~,~I_{1:S})] \\ 
    \text{s.t.}~T= \sum_{s=1}^{S} \frac{t_{s} \times N} {\lambda_s} ~ \le T_{budget} = \frac{T_{full}}{\lambda}, \nonumber
\end{align}
where $\mathcal{E}$ takes expectation over the images $I_{1:S}$ recovered from fully sampled data, $\mathcal{L}(\cdot,\cdot)$ is a loss function (say the $L_1$ loss we empirically use),  $T_{budget}$ is a given time budget, and $\lambda=T_{full}/T_{budget}$ is an overall time saving factor.

Unfortunately, directly solving the problem in (\ref{eq:recovery}) is challenging as it contains three subproblems related to (i) recovery model (RM), (ii) sampling ratio (SR), and (iii) sampling pattern (SP).
Specifically, 
\begin{itemize}
    \item 
The first RM subproblem is to select the right model $\mathcal{M}$ and optimize its associated parameter $\theta$, given a fixed sampling strategy with $\lambda_{1:S}$ and $\mathcal{G}_{1:S}$ known.
\item 
The second SR subproblem is to pick the right sampling ratio, that is, solving for $\lambda_{1:S}$ given a known model $\mathcal{M_{\theta}}$ and the best sampling pattern $\mathcal{G}_s$ for each sequence. In practice, choosing the right SR may also depend on the importance of each sequence with regards to specific diseases.
\item
The third SP subproblem is to select the right sampling pattern. Given a known model $\mathcal{M_{\theta}}$ and the desirable sampling ratios $\lambda_{1:S}$, we want to find the optimally efficient sampling pattern $\mathcal{G}_{1:S}$ that leads to the most information recovered for each sequence. 
\end{itemize}
To complicate the matter, the three subproblems are mixed together. The optimal recovery model depends on the sampling strategy and vice verse, while the best sampling pattern may be different for every sequence, under its specific sampling ratio.

In this paper, we make preliminary attempts with simplifying assumptions and empirical findings to solve these three subproblems. While we will touch on the effect of different SPs, the main focus of this paper will be on finding the best RM and SR with a pre-determined SP. 
%In general, we use sampling strategy (SS) as an umbrella term to mean variable SR and fixed SP. 



\subsection{Recovery network}
We use deep neural network (NN) as our choice for RM $\mathcal{M_{\theta}}$. Since the RM takes multiple images from different sequences as inputs, one has the choice of training (a) multiple individual NNs, one per sequence, or (b) one simultaneous, monolithic NN for all sequences. 

As mentioned above, the right RM choice might depend on the specific SR; however, we hypothesize that such an RM choice is independent of SR. This is realized by learning an RM that is insensitive to the SR. In other words, during the process of learning an RM, we take a data augmentation approach: for each training data point, we associate it with a random choice of $\lambda_{1:S}$.
We can then empirically verify which RM, individually or simultaneously learned, yield the smaller loss. 
\begin{align} \label{eq:RM}
    \min_{\mathcal{M_{\theta}} \in \mathcal{Z}}~~  \mathcal{L}_{recon} = \mathcal{E}_{p(I_{1:S},\lambda_{1:S})}[\mathcal{L}( \mathcal{M_{\theta}}(I_{\downarrow \lambda_{1:S}})~,~I_{1:S})],
\end{align}
where $\mathcal{Z}$ is the model zoo of interest and $\mathcal{E}$ takes expectation over the images $I_{1:S}$ recovered from fully sampled data and the sparsity factors $\lambda_{1:S}$. We denote the minimizing RM as $\tilde{\mathcal{M_{\theta}}}$.

\subsection{Sampling strategy}

Given the RM $\tilde{\mathcal{M_{\theta}}}$ learned in an SS-insensitive fashion and assuming that the sparsity factor $\lambda_s$ takes a value in a discrete set $\Lambda=\{\hat{\lambda}^1,\hat{\lambda}^2,...,\hat{\lambda}^F\}$, it is possible to find the optimal SS via exhaustive search. 

\begin{align} \label{eq:SS}
    \min_{\lambda_{1:S} \in \Lambda}~~  \mathcal{L}_{recon} = \mathcal{E}_{p(I_{1:S})}[\mathcal{L}( \tilde{\mathcal{M_{\theta}}}(I_{\downarrow \lambda_{1:S}})~,~I_{1:S})] \\ 
    \text{s.t.}~T= \sum_{s=1}^{S} \frac{t_{s} \times N} {\lambda_s} ~ \le T_{budget} = \frac{T_{full}}{\lambda}, \nonumber
\end{align}
where $\mathcal{E}$ takes expectation over the images $I_{1:S}$ recovered from fully sampled data.

This is done in two steps for each possible SS configuration.
\begin{itemize}
    \item Step 1: Check if the SS configuration satisfies the time constraint.
    \item Step 2: If it does, then compute its associated reconstruction loss. 
\end{itemize}
Out of all SS configurations that reaches Step 2, we pick the SS configuration that generates the minimal loss.

To further refine the reconstruction quality, we perform one final round of tuning by learning an RM model specific to the selected SS configuration or mutliples RMs corresponding to a list of top SS configurations.
\fi

% \subsubsection{Individual vs Simultaneous reconstruction}

% With many CNN-based MR reconstruction methods focused on single sequence reconstruction, a natural extension for multi-sequence scenario is to learn multiple models $\mathcal{M}_{\theta_1}, \mathcal{M}_{\theta_2},...,\mathcal{M}_{\theta_s}$, each of which focuses on de-alising noise for a specific sequence. In this case, the models together compose $\mathcal{M}_{\theta}$, and the overall reconstruction loss can written as 

% \begin{align}
%     \min_{\theta_s,\lambda_s}  \mathcal{L}_{recon} =  \mathcal{E}[\mathcal{L}(\{ \mathcal{M}_{\theta_s}(I_{\downarrow \lambda_s})\}_{s=1}^S~,~\{I_{s}\}_{s=1}^S)],
% \end{align}

% This formulation does not take into account the shared information across different sequences. As both Xiang et al. \cite{DBLP:conf/miccai/XiangCCZLWS18} and Huang et al. \cite{DBLP:conf/miccai/HuangCA12} have shown, there exist a large amount of correlation between sequences on the same patient, as they share the underlying anatomic structures. Even if some anatomic detail is lost in one sequence due to under-sampling, such information may be present in other sequences. On the other hand, this formulation also leads to training excessive amount of models, as the de-aliasing task is common over all sequences and will lead to network learning similar features. Therefore, it makes much more sense to train one network which has access to all the sequences, and let it learn the best features among them. In practice, 
















